Chance-Constrained AC Optimal Power Flow: Reformulations and Efficient Algorithms

Higher levels of renewable electricity generation increase uncertainty in power system operation. To ensure secure system operation, new tools that account for this uncertainty are required. In this paper, we formulate a chance-constrained AC optimal power flow problem, which guarantees that generation, power flows and voltages remain within their bounds with a pre-defined probability. We then propose an accurate, yet tractable analytical reformulation of the chance constraints. The reformulation maintains the full, non-linear AC power flow equations for the forecasted operating point, and models the impact of uncertainty through a linearization around this point. We discuss different solution algorithms, including one-shot optimization with and without recourse, and an iterative algorithm which enables scalable implementations. We further discuss how more general chance constraint reformulations can be incorporated within the iterative solution algorithm. In a case study based on four different IEEE systems, we compare the performance of the solution algorithms, and demonstrate scalability of the iterative scheme. We further show that the analytical reformulation accurately and efficiently enforces chance constraints in both in- and out-of-sample tests, and that the analytical approach outperforms two alternative, sample based chance constraint reformulations.

==> Approximate_AC_Chance_Constraints.tex <==
%\emph{In this chapter, we extend the \ac{ccopf} to a more accurate model involving the full AC power flow equations. 
%Due to the non-linearities and non-convexities of the AC power flow equations, the \ac{acopf} is a hard problem to solve, and trying to incorporate uncertainty makes it even harder. Particularly, modelling how uncertainties propagate throughout the system becomes more challenging when the relations are non-linear. 
%In the following, we propose a method based on partial linearization of the AC power flow equations, which allows for a reasonably accurate, yet computationally tractable representation of the system with uncertainty. First, we use the full AC power flow equations to obtain an accurate solution for the forecasted power injections. Second, assuming that the fluctuations are small compared to the total injections, we linearize the system around the forecasted operating point and model the impact of uncertainty based on the linearized system model. we then formulate a \ac{ccacopf} with chance constraints for active and reactive power generation, voltage and transmission limits. With the linearized uncertainty representation, we are able to apply the analytical chance constraint reformulation and obtain closed-form expressions for the chance constraints. 
%We further discuss different possibilities for solving the problem, including both a one-shot and an iterative solution approach.
%The iterative solution approach solves the chance-constrained problem as an outer iteration, which allows for a straightforward adaption of the method based on any existing AC OPF implementation.
%We demonstrate the probabilistic performance and scalability of the method in a case study, including simulations for four test systems ranging from the 24-bus IEEE RTS96 system to the Polish test case with 2383 buses. We further compare the proposed method based on linearization and analytical chance constraint reformulation with two alternative reformulations based on (i) a Monte Carlo simulation and (ii) the scenario approach for joint chance constraints. We find that the proposed method efficiently enforces the limit on constraint violations, while allowing for fast computation and a good cost-security trade-off.}

\iffalse
\section{Motivation and Related Work}
In this chapter, we propose a stochastic \ac{acopf} formulation with chance constraints to account for the impact of uncertainty. The AC power flow equations entail a more accurate model of the system, including losses and reactive power. This is of particular importance if we are interested in, e.g., distribution networks, where active and reactive power are strongly coupled, or system security, where AC feasibility is of key importance. The AC modelling allows us to include and probabilistically enforce a range of new constraints, such as voltage limits, reactive power constraints and power flow constraints based on apparent power or current magnitude. 

While chance constraints offer a comprehensive way of handling forecast uncertainty, it is generally challenging to reformulate the resulting OPF into a tractable optimization problem. In previous chapters and in the literature in general, \ac{ccopf} was typically based on DC power flow, which is easier to handle due to the linear relation between power flows and power injections. 
%Some chance-constrained formulations have however considered AC power flow, e.g. \cite{zhang2011, vrakopoulou2013AC, li2011, baker2016}, while other attempts to solve a stochastic \ac{acopf} include, e.g., the two-stage model in \cite{phan2014}. 
Different approximate algorithms for the \ac{ccacopf} have been suggested in, e.g, \cite{zhang2011}, where an iterative solution based on numerical integration and linearization of the AC power flow constraints is proposed, or \cite{li2011}, which employs an iterative approach based on the cumulant method and Cornish-Fischer expansion. 
Generally, many papers on \ac{ccacopf} utilize linearized versions of the AC power flow equations to obtain linear relationships between power injections, voltages and power flows. 
Examples include \cite{hojjat2015}, which solves a linearized \ac{ccacopf} to obtain optimal redispatch schedules, or \cite{baker2016}, which uses linearized equations to solve a voltage-constrained \ac{ccacopf} for a distribution network with PV in-feeds.
To the best of our knowledge, the most comprehensive \ac{ccacopf} formulation in terms of modelling the actual non-linear equations is provided in \cite{vrakopoulou2013AC}. In \cite{vrakopoulou2013AC}, the chance-constrained problem is formulated using a convex relaxation of the full AC power flow equations and a sample-based approach to handle the chance constraint. 
While this method guarantees feasibility of the chance constraints, computational tractability for large systems and ensuring that the resulting solution is actually physically meaningful (i.e., that the relaxation is exact) are still challenges to be addressed. 
All of the above approaches have only been applied to small test cases, signalling a need for approaches that are tractable for utility scale systems \cite{capitanescu2016}.


%In \cite{baker2016}, a voltage-constrained AC OPF with joint chance constraints is solved by robustifying the solution against an uncertainty set found through a Monte Carlo simulation. The approach is based on linearized AC power flow equations, and no transmission constraints are considered. 
%Ref. \cite{fang2014}, which employs a genetic algorithm and a Gram-Charlies approximation of the chance-constraint is employed.
%Check UC paper reference...
%CHECK CAPITANESCU PAPER FOR REFERENCES? Kyri Baker, probabilistic AC power flow (AEP methods) UMBRELLA!!!
%The approaches mentioned above have been applied only to small systems, signalling a need for approaches that are tractable for utility scale systems \cite{capitanescu2016}. %Further, several of the approximate approaches \cite{zhang2011, li2011} have limited ability to model reactions to the actual uncertainty realization, e.g., they cannot optimize the activation of reserves or corrective control as in the previous chapters. Finally, the linearization based methods \cite{} assume a certain the AC power flow equations are typically linearized around an assumed operating point, such both changes in the generation schedules and fluctuations contributes to inaccuracies as we move away from this point.

Here, we propose a method which is more accurate than a method based only on linearized equations. 
The proposed formulation of the \ac{ccacopf} is based on a partial linearization of the AC power flow formulation, where the forecasted operating point is represented through the full non-linear equations, and the impact of uncertainty is modelled by a linearization around this point. By keeping the full AC equations in the formulation, we ensure AC feasibility for the forecasted point. This is an improvement on previous linearization approaches, e.g. \cite{hojjat2015, baker2016}, where a change in scheduled generation and voltages away from the linearization point is only accounted for through the linearized equations, and is hence not guaranteed to be feasible. Further, assuming that the deviations are small compared to the overall power generation, the linearization around the expected point can be assumed to be a reasonably accurate representation. 
Similar ideas for linearization were applied to stochastic load flow in the 1970's, see \cite{dopazo1975} and discussion therein, and were also adopted in the risk-based OPF in \cite{fu2001}. 

With the suggested linearization technique, we keep the full non-linear dependence on generation and voltages at the expected operating point, but obtain a representation which is linear in the uncertain variables. The linear dependence allows us to apply the analytical chance constraint reformulation from Section \ref{sec:reformulation}, leading to closed-form expressions of the constraints. The accuracy of this chance constraint reformulation for apparent power flow constraints was first investigated in \cite{qu2015}, although without application in an optimization problem. Preliminary results for the application of the linearization approach to the \ac{ccacopf} problem were presented in \cite{schmidli2016}, including only parts of the model and limited testing on a small system.

Here, we present a more comprehensive model, including uncertainty of generator active and reactive power outputs. 
%including a proper model of generation uncertainty where we account for, e.g., adjustments of reactive power at PV buses. 
%Here, we both extend the modelling of generation uncertainty, accounting properly for adjustments of related to voltage control at PV buses and providing guarantees for the availability of reserve capacities. 
We further propose different solution algorithms for the problem, including 1) a one-shot optimization, which allows us to co-optimize reactions to the uncertainty realization, or 2) an iterative approach, which allows for integration with any existing \ac{acopf} solver and hence has significant potential for scalability and implementation in existing operating practices. 
The two solution methods are compared in terms of cost and computation time. We further demonstrate scalability by solving the \ac{ccacopf} problem for systems with up to 2383 buses.

Solving the \ac{ccacopf} using a linearization and analytical chance-constraint reformulation introduces two sources of inaccuracy, namely the linearization of the AC power flow equations and the assumption of the distributional parameters. Specifically, our case study assumes that the currents, votlages and generator outputs are normally distributed, as this was found to be a reasonable assumption for line flows in previous chapters. 
To assess the accuracy of the method, we run both in-sample Monte Carlo simulations to investigate approximation errors from the linearization, and out-of-sample tests to assess the overall performance. 

We further assess how well the analytical reformulation compares with two sample based reformulations. The first approach uses a Monte Carlo simulation to define empirical quantiles of the power flows. The second approach is based on the scenario approach \cite{campi2006, calafiore2006, campi2009}, and uses a pre-determined number of samples to define a worst-case margin that guarantees a maximum joint violation probability. 
We compare the three methods in terms of chance constraint feasibility, operational cost and computational time.
%We further compare the iterative solution scheme based on the analytical reformulation against a one-shot optimization, and show how the iterative algorithm can be used to scale the method to large systems. The one-shot solution is further extended to allow for co-optimization of the reserve participation vector $\alpha$, and the benefits of this additional degree of freedom are demonstrated. 
%Finally, the accuracy of the solution with respect to chance constraint satisfaction is assessed through a number of Monte Carlo simulations.
%We also assess how well the analytic reformulation compares to two sample based reformulations, the empirical margins computed with a Monte Carlo simulation and the constraint tightening obtained based on the scenario approach \cite{calafiore2006, campi2006, campi2009}. 
%Although the accuracy of the method reduces as the error size increases, 
%The introduced approximations are observed to provide good estimates for most chance constraints.

The remainder of the chapter is structured as follows. We first describe the AC OPF formulation with chance constraints and the approximate reformulation, before moving on to a description of the different solution approaches. 
Then a case study to assess the performance of the method is presented, before we summarize and conclude. 

The work presented in this chapter is extending the work performed in collaboration with Haoyuan Qu and Jeremias Schmidli during their semester theses work, which was documented in \cite{qu2014thesis, qu2015, schmidli2015thesis, schmidli2016}.


\section{Modelling Active and Reactive Power Uncertainty}
In this section, we present the modelling of active and reactive power deviations, as well as the reaction from conventional generators in order to maintain system balance and keep the voltage magnitudes at the chosen set-points.
To model generation and control at different types of buses, we distinguish between PQ, PV and $\theta V$ (reference) buses. We denote the sets of PQ, PV and $\theta$V buses by $\mathcal{N}_{PQ},~\mathcal{N}_{PV},~\mathcal{N}_{\theta V}\subset \mathcal{N}$, respectively. The number of PQ and PV buses is given by $|\mathcal{N}_{PQ}|=m_{PQ},~|\mathcal{N}_{PV}|=m_{PV}$. In our formulation, we assume only one $\theta V$ bus, although the method could be extended to account for a distributed slack bus. The sets $\mathcal{G}_{PQ},~\mathcal{G}_{PV},~\mathcal{G}_{\theta V}\subset \mathcal{G}$ represent generators connected at a PQ, PV and $\theta V$ buses. We denote variables at PQ buses by subscript $_{PQ}$, variables at PV buses by subscript $_{PV}$ and variables at the reference bus by subscript $_{\theta V}$.

\subsubsection{Uncertainty Modelling}
As explained in Section \ref{sec:uncertainty}, we can model the deviations in active power production as the sum of the forecasted production $u$ and a zero mean fluctuation $\omega$. We repeat the definition \eqref{eq:u_def3} here for convenience:
\begin{eqnarray}
    \tilde{u} = u + \omega~. \nonumber
\end{eqnarray}
When the active power production or consumption changes, it typically also impacts the reactive power injections. While the previously considered DC power flow formulations neglect reactive power, the AC power flow model requires a model for changes in the reactive power injections. 
Different models for reactive power might be applicable, depending on the type of uncertainty source (e.g., load or renewable generation). Here we choose to assume that the fluctuations have a \emph{constant power factor} $\cos \phi$, such that 
\begin{eqnarray}
    \tilde{q}_U = q_U + \gamma\omega~, \quad \text{where } \gamma = \sqrt{\frac{1-\cos^2 \phi}{\cos^2 \phi}}~. \nonumber
\end{eqnarray}
The variable $\gamma$ will be referred to as the power ratio in the following. 
Other possibilities to model reactive power deviations could assume, e.g., that the reactive power injections remain constant, that the reactive power can be dispatched (at least partially) independent of the active power production or that some uncertainty sources (e.g., large wind farms) participate in controlling the voltage at their point of connection. These types of control can be included in the formulation without any conceptual change. 

\subsubsection{Generation and Voltage Control}
In case of deviations from the scheduled reactive and active power injections, the controllable generators must control the produced reactive and active power in order to ensure power balance, and maintain the desired voltage profile.
For active power, we assume a similar set-up as in the DC case, where the power mismatch $\Omega$ is balanced through a centralized AGC signal as in \eqref{affine}. In addition to a direct mismatch in the power injections $\Omega$, the changes in power flows will also influence the system losses. We assume that the change in the active power losses, which is a-priori unknown and denoted by $\delta p$, is balanced out by the generator at the reference bus.
\begin{align}
    &\tilde{p}_{G,i}(\omega) = p_{G,i} - \alpha_i \Omega, \quad &&\forall_{i\in\mathcal{G}_{PQ},~\mathcal{G}_{PV}},\\
    &\tilde{p}_{G,i}(\omega) = p_{G,i} - \alpha_i \Omega + \delta p_i, \quad &&\forall_{i\in\mathcal{G}_{\theta V}},\\
    &\sum_{i\in\mathcal{G}}\alpha_i = 1.
\end{align}
For reactive power, we assume a more localized control. All generators connected at PV and $\theta$V buses change their outputs by $\delta q$ in order to keep voltage magnitudes constant. The generators connected at PQ buses do not change their output.
\begin{align}
    \tilde{q}_{G,i}(\omega) &= q_{G,i}, \quad &&\forall_{i\in\mathcal{G}_{PQ}}\\
    \tilde{q}_{G,i}(\omega) &= q_{G,i} + \delta q_i, \quad &&\forall_{i\in\mathcal{G}_{PV},~\mathcal{G}_{\theta V}}.
\end{align}
The change in voltage magnitudes can be expressed in a similar way. The voltage magnitude is fixed at the reference and PV buses, and changing in reaction to the uncertainty at PQ buses:
\begin{align}
    \tilde{v}_j(\omega) &= v_{j} + \delta v_j, \quad &&\forall_{j\in\mathcal{N}_{PQ}},\\
    \tilde{v}_j(\omega) &= v_{j},            \quad &&\forall_{j\in\mathcal{N}_{PV},~{N}_{\theta V}}.
\end{align}
Note that this type of local reactive power control only applies to how the generators react to the fluctuations $\omega$. The nominal reactive power dispatch of the generators, as well as the voltage set-points at PV and $\theta$V buses, are optimized as part of the OPF. We further remark that a centralized \ac{avr} scheme as in \cite{vrakopoulou2013AC}, with control variables similar to the participation factors $\alpha$ of the AGC, could also be implemented within the presented framework. 

\subsubsection{Power flows}
With deviations in the active and reactive power injections, the power flows throughout the system also change. Assuming a thermally constrained system, we model the power flows in terms of currents, with $i_{ij}$ representing the current magnitude on line $ij$. All currents are influenced by the uncertainty which induces a change $\delta i_{ij}$ in the current magnitude, 
\begin{align}
    \tilde{i}_{ij}(\omega) &= i_{ij} + \delta i_{ij}, \quad &&\forall_{ij\in\mathcal{L}}.
\end{align}

\section{Chance-Constrained AC Optimal Power Flow}
This section first presents the \ac{ccacopf}, discusses the interpretation of constraints, and points out why the problem in its original form is intractable. We then continue to explain how a tractable, approximate reformulation can be obtained, based on the full AC power flow for the nominal operating point and a linearization around that point for the deviations. %Finally, we comment on how the linearization factors are obtained.


\subsection{Original Problem}
%We first formulate the full \ac{ccacopf} problem. 
%We follow the notation from previous chapters, extended by reactive power $q$, voltage magnitude $v$ and angles $\theta$, as well as
We state the full \ac{ccacopf} as 
\begin{align}
\min_{p_G, q_G, v} ~~&  \sum_{i\in \mathcal{G}}\left(c_{2,i}p_{G,i}^2 + c_{1,i}p_{G,i} +c_{0,i}\right)&& \label{ac_obj}\\
% nodal power balance
\text{s.t.}  ~~         
&f\left( \tilde{\theta}(\omega), \tilde{v}(\omega), \tilde{p}(\omega),\tilde{q}(\omega) \right) = 0 ~~&&\forall_{\omega \in \mathcal{D}} \label{ac_powerbal}\\
% generation constraints
&\mathbb{P}(\tilde{p}_{G,i}(\omega) \leq p_{G,i}^{max})\geq 1-\epsilon_P, ~~&&\forall_{i\in\mathcal{G}} \label{ac_pMax}\\
&\mathbb{P}(\tilde{p}_{G,i}(\omega) \geq p_{G,i}^{min})\geq 1-\epsilon_P, ~~&&\forall_{i\in\mathcal{G}} \label{ac_pMin}\\
&\mathbb{P}(\tilde{q}_{G,i}(\omega) \leq q_{G,i}^{max})\geq 1-\epsilon_Q, ~~&&\forall_{i\in\mathcal{G}} \label{ac_qMax}\\
&\mathbb{P}(\tilde{q}_{G,i}(\omega) \geq q_{G,i}^{min})\geq 1-\epsilon_Q, ~~&&\forall_{i\in\mathcal{G}} \label{ac_qMin}\\
% voltage constraint
&\mathbb{P}(\tilde{v}_{j}(\omega) \leq v_{j}^{max})\geq 1-\epsilon_V, ~~&&\forall_{j\in\mathcal{N}} \label{ac_vMax}\\
&\mathbb{P}(\tilde{v}_{j}(\omega) \geq v_{j}^{min})\geq 1-\epsilon_V, ~~&&\forall_{j\in\mathcal{N}} \label{ac_vMin}\\
% current constraint
&\mathbb{P}(\tilde{i}_{ij}(\omega) \leq i_{ij}^{max})\geq 1-\epsilon_I, ~~&&\forall_{ij\in\mathcal{L}} \label{ac_iMax}\\
&\theta_{\theta V} = 0 \label{ac_ref} 
\end{align}
The objective \eqref{ac_obj} is to minimize the cost of active power generation, which is modelled through a quadratic cost objective where $c_2$, $c_1$ and $c_0$ are the quadratic, linear and constant cost coefficients\footnote{We use a quadratic objective, which is a generalization compared to the linear objectives used in the previous chapters. The quadratic objective is a more accurate model of the true cost of generation, and is particularly of interest when minimizing actual generation cost, as in a vertically integrated utility. A (piecewise) linear cost function is more representative for the bids from generators to a market operator, which must typically be provided in \$/MW.}. 
Eq. \eqref{ac_powerbal} are the nodal power balance constraints based on the full non-linear AC power flow constraints. These equations are functions of the nodal voltage angles $\tilde{\theta}(\omega)$ and magnitudes $\tilde{v}(\omega)$, as well as the nodal injections of active $\tilde{p}(\omega)$ and reactive power $\tilde{q}(\omega)$. The nodal power injections are the sum of the power injections from generator, loads and uncertainty sources,
\begin{align}
    &\tilde{p}(\omega) = \tilde{p}_G(\omega) + p_D + u + \omega, \\
    &\tilde{q}(\omega) = \tilde{q}_G(\omega) + q_D + q_U + \gamma\omega. 
\end{align}
%Their solution depends on the nodal injections of active power $\tilde{p}(\omega)$ and reactive power $\tilde{q}(\omega)$ and determines the nodal voltage angles $\tilde{\theta}(\omega)$ and magnitudes $\tilde{v}(\omega)$. 
Both the power injections and the nodal voltages depend on the realization of $\omega$, 
and the power balance constraints \eqref{ac_powerbal} must be maintained for all possible $\omega$ within the uncertainty set $\mathcal{D}$.
%and we enforce \eqref{ac_powerbal} for all possible $\omega$ within the uncertainty set $\mathcal{W}$.

The remaining constraints are generation constraints for active and reactive power \eqref{ac_pMax} - \eqref{ac_qMin}, constraints on the voltage magnitudes at each bus \eqref{ac_vMax}, \eqref{ac_vMin} and transmission constraints in the form of limits on the current magnitudes $\tilde{i}(\omega)$ \eqref{ac_iMax}. All these constraints are formulated as chance constraints with acceptable violation probabilities of $\epsilon_P,~\epsilon_Q, ~\epsilon_V$ and $\epsilon_I$, respectively. For the generation constraints, that are in reality hard constraints, a constraint violation would indicate a situation in which regular control actions would leave the system imbalanced and manual intervention would be needed, as explained in Section \ref{sec:first_genConstraints}. For the current and voltage constraints, a constraint violation would indicate an actual violation of the limit, which can either be tolerated or removed through additional control actions, analogous to the transmission limits on active power discussed in Section \ref{sec:first_transConstraints}.\\
Finally, the voltage angle at the reference bus is set to zero by \eqref{ac_ref}.

\subsection{Approximation of Uncertainty Impact}
The problem \eqref{ac_obj} - \eqref{ac_ref} is not tractable in its current form. First, it is not possible to directly enforce \eqref{ac_powerbal} for all $\omega$, as the set of fluctuations $\mathcal{D}$ is uncountable. Further, the chance constraints \eqref{ac_pMax}-\eqref{ac_iMax} must be reformulated into tractable constraints.
In the following, we present an approximate version of \eqref{ac_obj} - \eqref{ac_ref}, based on the following main idea: 
\begin{itemize}
    \item For the nominal operating point, given by $\omega = 0$ and the scheduled nodal power injections $p,~q$, we solve the full AC power flow equations. This allows us to get an accurate representation of the forecasted system state, and guarantees AC feasibility for the case without forecast errors.   
    \item The impact of the uncertainty $\omega$ is accounted for using a linearized representation of the system, based on Jacobian matrices evaluated at the nominal operating point. This modelling represents a first-order Taylor expansion around the nominal operating point, and can be assumed to be reasonably accurate when the fluctuations $\omega$ are small compared to the overall scheduled power injections $\mid \omega \mid << \mid \sum_{i\in\mathcal{N}}p_i \mid$.
\end{itemize}
Following the above ideas, we replace \eqref{ac_powerbal} by a single set of deterministic equations for the forecasted operating point,
\begin{equation}
    f\left( \theta, v, p, q \right) = 0, \label{nominal_OP}% \nonumber
\end{equation}
where $\theta,~v$ are the voltage angles and magnitudes corresponding to the scheduled injections.
Based on the operating point obtained from \eqref{nominal_OP}, we define sensitivity factors with respect to the fluctuations $\omega$, i.e.,
\begin{align}
    &\mathbf{\Gamma}_{P} = \left.\begin{array}{c}\frac{\partial p_G}{\partial \omega}\end{array} \! \right\vert_{(\theta, v, p, q)}, \quad
    &\mathbf{\Gamma}_{V} = \left.\begin{array}{c}\frac{\partial v}{\partial \omega} \end{array} \! \right\vert_{(\theta, v, p, q)}, 
    \nonumber\\
    &\mathbf{\Gamma}_{Q} = \left.\begin{array}{c}\frac{\partial q_G}{\partial \omega}\end{array} \! \right\vert_{(\theta, v, p, q)}, \quad
    &\mathbf{\Gamma}_{I} = \left.\begin{array}{c}\frac{\partial i}{\partial \omega} \end{array} \! \right\vert_{(\theta, v, p, q)}. 
    \nonumber
\end{align}
Here, $\mathbf{\Gamma}_P,~\mathbf{\Gamma}_Q$ denote the sensitivity factors for the active and reactive power injections, respectively, while $\mathbf{\Gamma}_V,~\mathbf{\Gamma}_I$ are the sensitivity factors for the voltage and current magnitudes. The sensitivity factors allow us to approximate the changes in the power injections $\delta p,~\delta q$ and the voltage and current magnitudes $\delta v,~\delta i$ as linear functions of $\omega$,
\begin{align}
    \tilde{p}_{G,i}(\omega) &= p_{G,i} + \delta p_i \approx p_{G,i} - \alpha_i\Omega + \mathbf{\Gamma}_{P(i,\cdot)} \omega, 
    && \forall_{i\in\mathcal{G}_{\theta V}} \nonumber\\
    \tilde{q}_{G,i}(\omega) &= q_{G,i} + \delta q_i \approx q_{G,i} + \mathbf{\Gamma}_{Q(i,\cdot)} \omega, 
    && \forall_{i\in\mathcal{G}_{\theta V}, \mathcal{G}_{P V}} \nonumber\\
    \tilde{v}_{j}(\omega)  &= v_{j} + \delta v_j \approx v_{j} + \mathbf{\Gamma}_{V(j,\cdot)} \omega, 
    && \forall_{j\in\mathcal{G}_{PQ}} \nonumber\\
    \tilde{i}_{ij}(\omega) &= i_{ij} + \delta i_{ij} \approx i_{ij} + \mathbf{\Gamma}_{I(ij,\cdot)} \omega.
    && \forall_{ij\in\mathcal{L}} \nonumber
\end{align}
The derivation of the sensitivity factors $\mathbf{\Gamma}_P,~\mathbf{\Gamma}_Q,~\mathbf{\Gamma}_V$ and $\mathbf{\Gamma}_I$ can be found in Appendix \ref{app:Appendix}. Here, we only note that they depend non-linearly on the forecasted operating point $p,~q,~v$ and $\theta$, and linearly on the participation factors $\alpha$ and the power ratio $\gamma$.

%This approximate reformulation allows us to reduce \eqref{ac_powerbal} to a single set of deterministic equations for the nominal operating point. It further enables the definition of linear sensitivity factors $\mathbf{\Gamma}$ to model the changes in generation, currents and voltages. The chance constraints can thus be expressed as the sum between a nominal value and a change which depends linearly on $\omega$. 

\subsection{Approximate AC CC-OPF}
With the above considerations, we can rewrite \eqref{ac_obj} - \eqref{ac_ref} in the following way:
%where the sets $\mathcal{N}_{PQ},~\mathcal{N}_{PV},~\mathcal{N}_{\theta V}\subset \mathcal{N}$ represent the sets of PQ buses, PV buses and $\theta$V buses, respectively. The sets $\mathcal{G}_{PQ},~\mathcal{G}_{PV},~\mathcal{G}_{\theta V}\subset \mathcal{G}$ represents generators connected at a PQ, PV or the reference bus. 
\begin{align}
\min_{p_G, q_G, v} ~~&  \sum_{i\in \mathcal{G}}\left(c_{2,i}p_{G,i}^2 + c_{1,i}p_{G,i} +c_{0,i}\right)& \label{ac_obj_ref}\\
% nodal power balance
\text{s.t.} ~~          
&f\left( \theta, v, p, q \right) = 0 ~~&& \label{ac_powerbal_ref}\\
% generation constraints
% active power
&\mathbb{P}(p_{G,i} - \alpha_i \Omega \leq p_{G,i}^{max})\geq 1-\epsilon_P, ~~&&\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ},~ \mathcal{G}_{PV}} \label{ac_pMax_refPQ}\\
&\mathbb{P}(p_{G,i} - \alpha_i \Omega \geq p_{G,i}^{min})\geq 1-\epsilon_P, ~~&&\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ},~ \mathcal{G}_{PV}} \label{ac_pMin_refPQ}\\
&\mathbb{P}(p_{G,i} - \alpha_i \Omega + \mathbf{\Gamma}_{P(i,\cdot)} \omega \leq p_{G,i}^{max})\geq 1-\epsilon_P,&& \forall_{i\in\mathcal{G}_{\theta V}} \label{ac_pMax_refTV}\\
&\mathbb{P}(p_{G,i} - \alpha_i \Omega + \mathbf{\Gamma}_{P(i,\cdot)} \omega \geq p_{G,i}^{min})\geq 1-\epsilon_P,&& \forall_{i\in\mathcal{G}_{\theta V}} \label{ac_pMin_refTV}\\
% reactive power
&q_{G,i}^{min} \leq q_{G,i} \leq q_{G,i}^{max}   ~~&&\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ}} \label{ac_q_refPQ}\\
&\mathbb{P}(q_{G,i} + \mathbf{\Gamma}_{Q(i,\cdot)} \omega \leq q_{G,i}^{max})\geq 1-\epsilon_Q, ~~&&\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PV},~\mathcal{G}_{\theta V}} \label{ac_qMax_refTV}\\
&\mathbb{P}(q_{G,i} + \mathbf{\Gamma}_{Q(i,\cdot)} \omega \geq q_{G,i}^{min})\geq 1-\epsilon_Q, ~~&&\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PV},~\mathcal{G}_{\theta V}} \label{ac_qMin_refTV}\\
% voltage constraint
&\mathbb{P}(v_{j}  + \mathbf{\Gamma}_{V(j,\cdot)} \omega \leq v_{j}^{max})\geq 1-\epsilon_V, ~~&&\!\!\!\!\!\!\!\!\forall_{j\in\mathcal{N}_{PQ}} \label{ac_vMax_refPQ}\\
&\mathbb{P}(v_{j}  + \mathbf{\Gamma}_{V(j,\cdot)} \omega \geq v_{j}^{min})\geq 1-\epsilon_V, ~~&&\!\!\!\!\!\!\!\!\forall_{j\in\mathcal{N}_{PQ}} \label{ac_vMin_refPQ}\\
&v_{j}^{min} \leq v_{j} \leq v_{j}^{max}   ~~&&\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{N}_{PV},~\mathcal{N}_{\theta V}} \label{ac_v_refPV}\\
% current constraint
&\mathbb{P}(i_{ij} + \mathbf{\Gamma}_{I(ij,\cdot)} \omega \leq i_{ij}^{max})\geq 1-\epsilon_I, ~~&&\!\!\!\!\!\!\!\!\forall_{ij\in\mathcal{L}} \label{ac_iMax_ref}\\
&\theta_{\theta V} = 0 \label{ac_ref_ref} 
\end{align}
Note that the active power chance constraints \eqref{ac_pMax_refTV}, \eqref{ac_pMin_refTV} for the $\theta V$ bus depends on $\mathbf{\Gamma}_P$, while the reactive power chance constraint for the PV and $\theta V$ buses depend on $\mathbf{\Gamma}_Q$. The reactive power constraints for the PQ buses \eqref{ac_q_refPQ} are deterministic, as the power injections are fixed.
Similarly, the chance constraints on the voltage magnitudes at PQ buses \eqref{ac_vMax_refPQ}, \eqref{ac_vMin_refPQ} are chance constraints which depend on $\mathbf{\Gamma}_V$, whereas the voltage magnitude constraints for the reference and PV buses are deterministic.
All current constraints \eqref{ac_iMax_ref} are chance constraints, with the dependency on $\omega$ expressed through $\mathbf{\Gamma}_I$. Note that the forecasted current magnitude $i_{ij}$ is a function of the full non-linear AC power flow equations.

%The objective \eqref{ac_obj_ref} remains unchanged, while \eqref{ac_powerbal_ref} represents the nominal power flows in the system.
%The generation constraints for active power \eqref{ac_pMax_refPQ}, \eqref{ac_pMin_refPQ} incorporate both the scheduled operating point and the activation of active power through the \ac{agc} signal. 
%The constraints for active power at the reference bus \eqref{ac_pMax_refTV}, \eqref{ac_pMin_refTV} contain the additional term $\mathbf{\Gamma}_{G,i} \omega$, which is a linearized representation of the change in system losses $\delta p$.
%The reactive power constraints at PQ buses \eqref{ac_q_refPQ} are deterministic, since the reactive power injections are fixed at their nominal value $q_G$. At the reference and PV buses, the dependency on $\omega$ gives rise to the chance constraints \eqref{ac_qMax_refTV}, \eqref{ac_qMin_refTV}. 
%Similarly, the chance constraints on the voltage magnitudes at PQ buses are formulated as chance constraints \eqref{ac_vMax_refPQ}, \eqref{ac_vMin_refPQ}, whereas the voltage magnitude constraints for the reference and PV buses are deterministic. %, since the magnitudes are fixed at the nominal value $v_j$.
%Finally, the current constraints \eqref{ac_iMax_ref} are formulated as chance constraints. Note that the nominal current magnitude $i_{ij}$ is a function of the full non-linear AC power flow equations.

\subsection{Chance Constraint Reformulation}
%By approximating the changes in power injections, voltage magnitudes and currents as the product between a sensitivity factor $\mathbf{\Gamma}_P,~\mathbf{\Gamma}_Q,~\mathbf{\Gamma}_V$ and $\mathbf{\Gamma}_I$ and $\omega$, the chance constraints \eqref{ac_pMax_refPQ} - \eqref{ac_pMin_refTV}, \eqref{ac_qMax_refTV} - \eqref{ac_vMin_refPQ} and \eqref{ac_iMax_ref} all depends linearly on the uncertain variable $\omega$.
%With the definition of the sensitivity factors $\mathbf{\Gamma}_P,~\mathbf{\Gamma}_Q,~\mathbf{\Gamma}_V$ and $\mathbf{\Gamma}_I$, the chance constraints \eqref{ac_pMax_refPQ} - \eqref{ac_pMin_refTV}, \eqref{ac_qMax_refTV} - \eqref{ac_vMin_refPQ} and \eqref{ac_iMax_ref} all depends linearly on $\omega$.
In the above formulation, the chance constraints are linear functions of $\omega$. This implies that we can use the analytical reformulation as in section \ref{sec:reformulation}. This reformulation is applicable whenever we have a linear dependency on the uncertain variables, even though the sensitivity factors $\mathbf{\Gamma}_P,~\mathbf{\Gamma}_Q,~\mathbf{\Gamma}_V,~\mathbf{\Gamma}_I$ are or the current magnitudes $i_{ij}$ are non-linear functions of the decision variables. 

Using this reformulation, we can express \eqref{ac_obj_ref} - \eqref{ac_ref_ref} as
\begin{align}
\min_{p_G, q_G, v} ~&  \sum_{i\in \mathcal{G}}\left(c_{2,i}p_{G,i}^2 + c_{1,i}p_{G,i} +c_{0,i}\right)&  \label{eq1}\\
% nodal power balance
\text{s.t.} ~          
&f\left( \theta, v, p, q \right) = 0 
~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{\omega \in \mathcal{D}}  \label{eq2}\\
% generation constraints
% active power
&p_{G,i} +\! \alpha_i f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_P)\sigma_\Omega \leq p_{G,i}^{max}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ},~ \mathcal{G}_{PV}}  \label{eq3}\\
&p_{G,i} -\! \alpha_i f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_P)\sigma_\Omega \geq p_{G,i}^{min}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ},~ \mathcal{G}_{PV}}  \label{eq4}\\
&p_{G,i} +\! f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_P) \!\parallel\! \Sigma_W^{1/2} (-\alpha_i \mathbf{1}_{1,m} + \mathbf{\Gamma}_{P(i,\cdot)})^T \!\!\parallel_2 \leq p_{G,i}^{max},\!\!\!\! &&\forall_{i\in\mathcal{G}_{\theta V}} \label{eq5}\\
&p_{G,i} -\! f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_P) \!\!\parallel\! \Sigma_W^{1/2} (-\alpha_i \mathbf{1}_{1,m} + \mathbf{\Gamma}_{P(i,\cdot)})^T \!\!\parallel_2 \geq p_{G,i}^{min},\!\!\!\! &&\forall_{i\in\mathcal{G}_{\theta V}} \label{eq6}\\
% reactive power
&q_{G,i}^{min} \leq q_{G,i} \leq q_{G,i}^{max}   
~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ}} \label{eq7}\\
&q_{G,i} + f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_Q) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{Q(i,\cdot)}^T \!\parallel_2 \leq q_{G,i}^{max}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PV},~\mathcal{G}_{\theta V}} \label{eq8}\\
&q_{G,i} - f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_Q) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{Q(i,\cdot)}^T \!\parallel_2 \geq q_{G,i}^{min}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PV},~\mathcal{G}_{\theta V}} \label{eq9}\\
% voltage constraint
&v_{j} + f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_V) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{V(j,\cdot)}^T \!\parallel_2 \leq v_{j}^{max}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ}}  \label{eq10}\\
&v_{j} - f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_V) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{V(j,\cdot)}^T \!\parallel_2 \geq v_{j}^{min}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ}}  \label{eq11}\\
&v_{j}^{min} \leq v_{j} \leq v_{j}^{max}   
~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{N}_{PV},~\mathcal{N}_{\theta V}}  \label{eq12}\\
% current constraint
&i_{ij} + f_{\mathcal{P}}^{-1}(1\!-\!\epsilon_I) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{I(ij,\cdot)}^T\!\parallel_2 \geq i_{ij}^{max}, ~~&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{ij\in\mathcal{L}}  \label{eq13}\\
&\theta_{\theta V} = 0 \label{eq14}
\end{align}
As for the previous chance-constrained formulations, we observe that the consideration of uncertainty introduce a similar uncertainty margin, i.e., a tightening of the nominal constraints. The uncertainty margins for active and reactive power are defined by
\begin{align}
    & \lambda_{P,i} = \alpha_i f_{\mathcal{P}}^{-1}(1-\epsilon_P)\sigma_\Omega,
    &&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PQ},~ \mathcal{G}_{PV}}, \label{uncP}\\
    & \lambda_{P,i} =  f_{\mathcal{P}}^{-1}(1-\epsilon_P) \!\parallel\! \Sigma_W^{1/2} (-\alpha_i \mathbf{1}_{1,m} + \mathbf{\Gamma}_{P(i,\cdot)})^T \!\parallel_2, &&\forall_{i\in\mathcal{G}_{\theta V}}, \\
    & \lambda_{Q,i} = f_{\mathcal{P}}^{-1}(1-\epsilon_Q) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{Q(i,\cdot)}^T \!\parallel_2,
    &&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\forall_{i\in\mathcal{G}_{PV},~ \mathcal{G}_{\theta V} },
\end{align}
while the voltage and current margins are given by
\begin{align}
    & \lambda_{V,j} = f_{\mathcal{P}}^{-1}(1-\epsilon_V) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{V(j,\cdot)}^T \!\parallel_2
    &&\forall_{j\in\mathcal{N}_{PQ}} \label{uncV}, \\
    & \lambda_{I,ij} =  f_{\mathcal{P}}^{-1}(1-\epsilon_I) \!\parallel\! \Sigma_W^{1/2} \mathbf{\Gamma}_{I,i}^T \!\parallel_2 &&\forall_{ij\in\mathcal{L}}. \label{uncI}
\end{align}
The general function $f_{\mathcal{P}}$ is used to emphasize that we can apply either of the five analytical reformulations in Table \ref{tableI}. %Since the AC power flow equations are non-linear, and it is not clear how the uncertainty propagates through the system, it might be of particular interest to use a more general uncertainty assumption, such as, e.g., unimodality. 


\section{Solution Algorithms}
In the following, we discuss two ways of solving the approximate \ac{ccacopf} formulated above. 

\subsection{One-Shot Optimization} 
The reformulated \ac{ccacopf} given by \eqref{eq1} - \eqref{eq14} is a continuous, non-convex optimization problem. 
The most obvious way to find a solution is therefore to pass the entire problem to a suitable solver. 
The solver will optimize the generation dispatch, while inherently accounting for the dependency of the sensitivity factors on the current nominal point $p,~q,~v,~\theta$ and the participation factors $\alpha,~\gamma$. 
By including $\alpha$ and $\gamma$ as optimization variables, it is thus possible to optimize not only the nominal dispatch, but also the reaction to fluctuations. Note that the problem is not guaranteed to converge to a global optimum, as it is non-convex.

The drawback of attempting a one-shot solution is the problem complexity, which might lead to long solution times.
%and little knowledge about the quality of the obtained solution. 
The deterministic \ac{acopf} is already a non-convex problem, and adding additional terms with complex dependencies on the decision variables only increases the difficulty of solving the problem. This can be a bottleneck for adoption in more realistic settings, where scalability and robustness of the solutions are important criteria. 
%Even when a solution is obtained, the solver only guarantees local optimality. 
%Recent work on convex relaxations of the deterministic \ac{acopf} [Dan, etc.] allows us to find globally optimal solutions, assess the maximum optimality gap for solutions obtained with other algorithms or prove infeasibility of a problem. Understanding what glob

\subsection{Iterative Solution Algorithm}
\label{sec:iterative}
To address the problem of increased computational complexity, we propose an iterative solution algorithm which allows us to solve the \ac{ccacopf} using any existing \ac{acopf} tool. 
For example, the iterative algorithm can utilize convex relaxations of the deterministic \ac{acopf} to find globally optimal solutions for the nominal operating point, or be added as an outer loop on AC OPF implementations already available in industry. This facilitates adoption into existing processes, and allows the algorithm to take advantage of previous efforts to increase robustness and scalability of the underlying \ac{acopf} tool. 
%A related algorithm was implemented as part of the security assessment tool box developed within the UMBRELLA project,  

The iterative solution algorithm is based on the observation that the uncertainty only occurs in the uncertainty margins defined by \eqref{uncP} - \eqref{uncI}. Assume that the participation factors $\alpha$ for the \ac{agc} and the power ratio $\gamma$ of the uncertain power injections are known. Then, for a given operating point, the uncertainty margins can be pre-calculated, and the \ac{ccacopf} can be solved as a standard \ac{acopf} with limits adjusted by the uncertainty margin:
\begin{align}
    & p_G^{min} + \lambda_P \leq p_G \leq p_G^{max} - \lambda_P \\
    & q_G^{min} + \lambda_Q \leq q_G \leq q_G^{max} - \lambda_Q \\
    & v^{min} + \lambda_V \leq v \leq v^{max} - \lambda_V \\
    & i \leq i^{max} - \lambda_I 
\end{align}
However, the linearization point $(\theta,v,p,q)$ is not known a-priori. 
Therefore, we solve the problem using an iterative approach, which uses the maximum change of the uncertainty margins (between subsequent iterations) as a measure of convergence. The approach consist of the following steps:
\begin{enumerate}
\item \emph{Initialization:} Set uncertainty margins $\lambda_P^0=\lambda_Q^0=\lambda_V^0=\lambda_I^0=0$, and iteration count $\kappa=0$.
\item \emph{Solve AC OPF:} Solve the AC OPF defined by \eqref{eq1} - \eqref{eq14}, and increase iteration count $\kappa=\kappa+1$.
\item \emph{Evaluate uncertainty margins:} Compute the uncertainty margins of the current iteration $\lambda_P^{\kappa},~\lambda_Q^{\kappa},~\lambda_V^{\kappa}$ and $\lambda_I^{\kappa}$, and evaluate the maximum difference to the last iteration for the power injections, voltages and currents,
\begin{align}
    & \eta^{\kappa}_P = \max\{|\lambda_P^{\kappa}-\lambda_P^{\kappa-1}|\}~, \quad\quad
     \eta^{\kappa}_Q = \max\{|\lambda_Q^{\kappa}-\lambda_Q^{\kappa-1}|\}~,\nonumber\\
    & \eta^{\kappa}_V = \max\{|\lambda_V^{\kappa}-\lambda_V^{\kappa-1}|\}~, \quad\quad
     \eta^{\kappa}_I = \max\{|\lambda_I^{\kappa}-\lambda_I^{\kappa-1}|\}~.\nonumber
\end{align}
%$\eta^{\kappa}_P = \max\{|\lambda_P^{\kappa}-\lambda_P^{\kappa-1}|\}$, $\eta^{\kappa}_Q = \max\{|\lambda_Q^{\kappa}-\lambda_Q^{\kappa-1}|\}$, voltages $\eta^{\kappa}_V = \max\{|\lambda_V^{\kappa}-\lambda_V^{\kappa-1}|\}$ and currents $\eta^{\kappa}_I = \max\{|\lambda_I^{\kappa}-\lambda_I^{\kappa-1}|\}$.
\item \emph{Check convergence:} If the maximum difference is small enough, stop.
\begin{equation}
        \eta_P^{\kappa}\leq\hat{\eta}_P~, \quad
        \eta_Q^{\kappa}\leq\hat{\eta}_Q~, \quad
        \eta_V^{\kappa}\leq\hat{\eta}_V~, \quad
        \eta_I^{\kappa}\leq\hat{\eta}_I~. \nonumber
\end{equation}
%$\eta_P^{\kappa}\leq\hat{\eta}_P$, $\eta_Q^{\kappa}\leq\hat{\eta}_Q$, $\eta_V^{\kappa}\leq\hat{\eta}_V$ and $\eta_I^{\kappa}\leq\hat{\eta}_I$, stop. 
If not, move back to step 1.
\end{enumerate}
The accuracy of the solution is defined through the choice of the stopping criteria $\hat{\eta}_P,~\hat{\eta}_Q,~\hat{\eta}_V$, and $\hat{\eta}_I$.

While the above algorithm is straight forward to implement, it has some drawbacks:

First, the uncertainty margins can only be computed as part of the outer loop, which takes the forecasted operating point and values for $\alpha$ and $\gamma$ as inputs. 
Since the uncertainty margins are not part of the inner loop optimization, the iterative \ac{ccacopf} does not define the operating point, $\alpha$ or $\gamma$ in a way that minimizes the uncertainty margins on congested lines or on buses with tight voltage constraints. 
%Hence, the iterative approach does not account for the influence of $\alpha$ and $\gamma$ on power flows or voltage magnitudes. 
It is however possible to include the influence of $\alpha$ on the generation dispatch by keeping $\alpha$ as a variable in the generation constraints \eqref{eq3} - \eqref{eq6}.
%CAN GAMMA BE DETERMINED USING AN OPTIMIZATION PROBLEM??? Further, since $\gamma$ only appears in the uncertainty margin, it would be possible to formulate the definition of $\gamma$ as an optimization pro

Second, the solution is not guaranteed to converge. 
In our simulations, the algorithm converged within a few iterations when $\hat{\eta}_P,~\hat{\eta}_Q,~\hat{\eta}_V$ and $\hat{\eta}_I$ are chosen not smaller than 0.001 MVA for active and reactive power, and $10^{-5}$ p.u. for voltage and current magnitudes.
%in the order of 0.001 MVA (when $\alpha$ is predefined) or 0.1 MVA (when $\alpha$ is an optimization variable) for active and reactive power, and or $10^{-5}$ p.u. for voltage and current magnitudes.
However, we observed that when the stopping criteria $\hat{\eta}_P,~\hat{\eta}_Q,~\hat{\eta}_V$, and $\hat{\eta}_I$ are chosen to be even smaller, the solution does not settle. Instead, each iteration finds a slightly different solution in the vicinity of the optimum.

However, the main change in the solution occurs between the first and second iterations, where the uncertainty margins increase from zero to the value corresponding to the optimal point of the deterministic \ac{acopf}. Even in case of non-convergence, stopping the algorithm after a given number of iterations and choosing the solution corresponding to the smallest change $\eta^{\kappa}_P,~\eta^{\kappa}_Q,~\eta^{\kappa}_V,~\eta^{\kappa}_I$ between iterations should, in most cases, provide a reasonable approximation of the true solution to the chance-constrained problem.

%First, it does not account for the influence of $\alpha$ and $\gamma$ on power flows or voltage magnitudes. It would however be possible to include the influence of $\alpha$ on the generation dispatch and reserve allocation, by keeping $\alpha$ as a variable in \eqref{eq3} - \eqref{eq6}. 
%Second, the solution is not guaranteed to converge. In particular, if the stopping criteria $\hat{\eta}_P,~\hat{\eta}_Q,~\hat{\eta}_V$, and $\hat{\eta}_I$ are chosen to be very small, the solution will continue to move around in the vicinity of the optimum. 
%However, it should be noted that for reasonable values of $\hat{\eta}_P,~\hat{\eta}_Q,~\hat{\eta}_V$, and $\hat{\eta}_I$ in the order of xx MVA or xx p.u., the algorithm was observed to converge within five iterations. 
%Further, the main change in the solution occurs between the first and second iterations, where the uncertainty margins increase from zero to the value corresponding to the optimal point of the deterministic \ac{acopf}. This implies that in case of non-convergence, stopping the algorithm after a given number of iterations and choosing the solution corresponding to the smallest change between iterations provides a good approximation of the true chance constraints.

\subsection{Alternative Iterative Solution Algorithms}
\label{sec:alternative}
When solving the problem using the iterative approach, the uncertainty margins $\lambda_P^{\kappa},~\lambda_Q^{\kappa},~\lambda_V^{\kappa}$ and $\lambda_I^{\kappa}$ are calculated only in the outer iteration. This opens for the possibility of using other methods than the analytical reformulation to calculate the uncertainty margins. 

\subsubsection{Empirical Uncertainty Margins from Monte Carlo Simulation}
One possibility is to define empirical uncertainty margins based on a Monte Carlo simulation. The uncertainty margins \eqref{uncP} - \eqref{uncI} represent an approximation of the quantile of the distribution of the currents, voltages and power generation. By sampling the uncertainty vector $\omega$ and calculating the resulting power flows for a large number of samples, we can compute empirical uncertainty margins $\lambda_P^{u,l},~\lambda_Q^{u,l},~\lambda_V^{u,l}$ and $\lambda_I^{u,l}$. 

For example, assume we want to ensure a voltage magnitude constraint with $\epsilon_V=0.01$ and use 1000 samples of $\omega$. To compute the upper and lower quantiles, we run the power flow for each sample. The upper quantile corresponds to the $10^{th}$ largest magnitude $v_{j}^{10}$, and the lower quantile to the $10^{th}$ lowest magnitude $v_{j}^{990}$. The upper and lower uncertainty margins are defined by $\lambda_V^{u} = v_{j}^{10} - v_{j}$ and $\lambda_V^{l} = v_{j} - v_{j}^{990}$, respectively. Note that the empirical uncertainty margins are not necessarily symmetric due to the non-linearity of the AC power flow equations. 

A similar Monte Carlo approach to define the uncertainty margins was implemented as part of the prototype toolbox in the UMBRELLA project \cite{morales2016}, were it was shown to significantly reduce the probability of constraint violations. However, the implemented approach calculated the uncertainty margins based only on the forecasted operating point, and did not include any subsequent updates. 
Since the outcome of the Monte Carlo simulation and hence the uncertainty margins depend on the solution to the \ac{acopf} for the forecasted operating point, we implement the Monte Carlo based approach as part of the iterative framework. 

\subsubsection{Enforcing Joint Chance Constraints}
While the uncertainty margins \eqref{uncP} - \eqref{uncI} represent the quantiles of the respective constraints, they can more generally be understood as a tightening which is necessary to secure the system against uncertainty. 
A similar constraint tightening can be observed in other stochastic and robust formulations of the OPF problem. One example is the \ac{ccopf} formulations based on joint chance constraints, in e.g. \cite{vrakopoulou2012, vrakopoulou2013AC}.

In \cite{vrakopoulou2013AC}, the stochastic AC OPF is solved as a joint chance-constrained problem. The AC power flow equations are represented using a convex SDP relaxation \cite{bai2008}, and solved as a robust problem. The robust uncertainty set is defined by the method in \cite{margellos2014}, and represented in the AC OPF using the set vertices, defined as the maximum and minimum realizations of the observed variables. 

Another way of guaranteeing chance constraint feasibility is using the scenario approach \cite{calafiore2006, campi2006}, which defines a number of randomly drawn samples $N_S$ for which the system must remain within bounds. The number of samples is related to the decision variables $N_X$ and the acceptable joint violation probability $\epsilon_J$, and is given by \cite{campi2009}
\begin{equation}
        N_S \geq \frac{2}{\epsilon_J}\left(\ln\frac{1}{\beta} + N_X \right).
\end{equation}
The value $1-\beta$ represents the confidence level for satisfying the chance constraint, and can be chosen to be very small. 
By enforcing the system constraints for all samples, it is guaranteed that the system remains jointly secure with the desired probability. 
%One example is the \ac{ccopf} with joint chance constraints in \cite{vrakopoulou2012}. In this paper, the scenario approach \cite{calafiore2006, campi2006, campi2009} is used to define a number of samples $N_S$ for which the system must remain within bounds. The number of samples is related to the decision variables $N_X$, and is given by \cite{campi2009}
%\begin{equation}
%        N_S \geq \frac{2}{\epsilon}\left(\ln\frac{1}{\beta} + N_X \right).
%\end{equation}
%Here, $\beta$ represents the confidence level of satisfying the chance constraint. 
%By enforcing the system constraints for all samples, it is guaranteed that the system remains jointly secure with the desired probability. 

Representing uncertainty sets based on samples, or representing a robust set through the vertices as in \cite{vrakopoulou2013AC}, only applies when the underlying problem is convex, since convexity guarantees that the linear combination of feasible points remain within the convex, feasible set. 
%The scenario approach only applies when the underlying problem is convex. A related method proposed in \cite{margellos2014} uses the scenario approach to define an uncertainty set which contains at least the desired probability mass. The \ac{ccopf} problem can then be recast as a robust problem, as in \cite{vrakopoulou2013, vrakopoulou2013AC, margellos2013}.
The convex relaxation is hence necessary for the approach in \cite{vrakopoulou2013AC} to guarantee chance constraint feasibility. However, the relaxation itself is not guaranteed to be AC feasible, but might provide solutions that are not physical solutions to the power flow problem. 

Here, we take a slightly different approach. We solve the full, non-convex \ac{acopf} for the forecasted operating point, ensuring that we find a physically meaningful solution
%
\footnote{The \ac{acopf} for the forecasted operating point can be solved using a convex relaxation, as long as we ensure feasibility of the resulting solution and apply a tighter relaxations, such as the higher-order moment relaxation in \cite{molzahn2014, molzahn2015}, if the initial solution is not exact.}. 
%
We then draw a finite number of samples for which the solution should remain secure, as prescribed by the scenario approach \cite{campi2009}. While the scenario approach is not directly applicable to non-convex problems, we justify our approach by the fact that we only evaluate the samples in the vicinity of a local optimum, where the problem can be assumed to be locally convex. 
%For the iterative approach, we choose to use the original scenario approach which is based on a finite number of samples, as opposed to an uncertainty set. 
%While the scenario approach is not directly applicable to non-convex problems, we justify our approach by the fact that we only evaluate the samples in the vicinity of a local optimum, where the problem is locally convex. 

Assuming that the fluctuations $\omega$ are small enough for us to stay within this locally convex region, we run a power flow simulation for each of the $N_S$ scenarios. Based on the results, we find the two limiting scenarios for each constraint,
\begin{equation}
        v_{j}^{u}=\max\{v_{j}^m,~m=1,...,n_S\} \quad \text{and} \quad v_{j}^{l}=\min\{v_{j}^m,~m=1,...,n_S\} \nonumber
\end{equation}
i.e., the scenarios that lead to the highest and lowest flows.
We then define the upper and lower uncertainty margins as $\lambda_V^{u} = v_{j}^{u} - v_{j}$ and $\lambda_V^{l} = v_{j} - v_{j}^{l}$, and solve the problem again. 

\begin{figure}%[!t]
\includegraphics[width=0.95\columnwidth]{UncertaintyMarginsPlot_v3.eps}
\centering
\caption{Uncertainty margins $\lambda_{V,j}^u$, $\lambda_{V,j}^l$ for an example voltage constraint, as obtained with a given set of samples. The black line represents the forecasted voltage, and the histogram shows the empirical voltage distribution for the given sample set. From top to bottom, we see the uncertainty margins obtained with the analytical reformulation, with a Monte Carlo simulation and with the scenario approach. }
\label{UncMargDemo} 
\end{figure}

As for the other iterative approaches, the computation of $v_{j}^u$ and $v_{j}^l$ depends on the solution obtained with the \ac{acopf} for the forecasted operating point. The iterations hence continue until the uncertainty margins have converged. With the final solution, where none of the samples are violated, the problem is guaranteed to have a joint violation probability below the prescribed value. 
%As for the other iterative approaches, the uncertainty margins depends on the nominal operating point. The problem should therefore be solved in an iterative fashion, with an update of the uncertainty margins in each iteration, to ensure that the final solution is feasible for all samples. 



A comparison of the three approaches to define uncertainty margins is shown for an example voltage constraint in Fig. \ref{UncMargDemo}. The histogram represents the empirical distribution of the voltage magnitudes, as calculated based on the samples used in the Monte Carlo simulation and the scenario approach. The analytical margins (top) are calculated based on \eqref{uncV} with a normal distribution assumption, the Monte Carlo margins (middle) correspond to the empirical margin of the given set of samples, and the scenario approach (bottom) uses the extreme scenarios to define the margins.
We observe that the analytical margins are symmetric, which in this case leads to a slight overestimation of the upper margin and a slight underestimation of the lower margin compared with the empirical Monte Carlo margins. The difference is however very small, although the underlying samples are not normally distributed. Further, we see that the scenario approach has much larger uncertainty margins than either of the two other approaches, as it only depends on the worst among the drawn scenarios. However, it should also be noted that the uncertainty margins for the scenario approach are not directly comparable to the uncertainty margins for the analytical and Monte Carlo approach. In this example, the number of samples in the scenario approach was chosen to guarantee a joint violation probability of $\epsilon_J\leq0.1$, whereas the uncertainty margins of the analytical and Monte Carlo reformulations aim at limiting the violation probability of each constraint to $\epsilon\leq0.01$. 



%While the general scenario approach is only applicable to convex optimization problems, a related approach proposed in \cite{margellos2014} is applicable also when the underlying problem is non-convex \cite{margellos2013}. By following the approach in \cite{margellos2014}, it is possible to define a set of uncertainty samples for which the system needs to be secure in order to guarantee that the joint violation probability remains below the desired level. Taking the 

\section{Case Study}
In the following, we study the performance of the approximate \ac{ccacopf}. We first investigate the different solution algorithms in terms of nominal operating cost and computational complexity, and demonstrate scalability of the iterative approach. We continue with an assessment of the performance of the approximate chance constraint reformulation. We perform both in-sample and out-of-sample testing, and compare the iterative approach based on analytic uncertainty margins with the iterative approaches based on Monte Carlo simulations and the scenario approach. 

\subsection{Test systems}
We run simulations for four different test systems, as described below. As a base case, we enforce all chance constraints with violation probabilities $\epsilon_P = \epsilon_Q = \epsilon_V = \epsilon_I = 0.01$. 
We assume that uncertainty from load and renewable generation is observed as fluctuations in the net load. The number of uncertain loads and their respective standard deviations are chosen to obtain congested, but feasible test cases. 
For the analytical reformulation, we assume that $\omega$ follows a multivariate normal distribution. 
For the iterative solution algorithms we set $\hat{\eta}_P=\hat{\eta}_Q=0.001 MVA$, $\hat{\eta}_V=10^{-5} p.u.$ and $\hat{\eta}_I=0.001 kA$.
%
\subsubsection{IEEE RTS96 One Area Test Case}
We base our test case on the data for the RTS96 system provided with Matpower 5.1 \cite{zimmermann2011}. We do not consider unit commitment, and hence set the lower limit on the generator ouput to zero. To obtain an interesting case, the generation limits are increased by a factor of 1.5. All 17 loads are assumed to be uncertain, with standard deviations equal to 10\% of the forecasted consumption and zero correlation between loads. 
%
\subsubsection{IEEE 118 Bus Test System}
We use a modified version of the 118 bus system included in the NICTA Energy System Test Archive \cite{coffrin2014}. For similar reasons as above, we set the lower generation limit to zero and increase the upper limit by a factor of 1.5. The 99 loads are all assumed to be uncertain, with standard deviations equal to 5\% of their forecasted consumption. The 118 bus system is split into three zones as described in Section \ref{test_system_118_corrective}, and we assume a correlation coefficient $\rho=0.3$ between loads within one zone, and zero correlation between loads in different zones. 
%
\subsubsection{IEEE 300 Bus Test System}
We use IEEE 300 bus test system included in the NICTA Energy System Test Archive \cite{coffrin2014}, with the lower generation limit to zero. The loads with consumption between 0 and 100 MW are assumed to be uncertain, with standard deviations equal to 5\% of their forecasted consumption and zero correlation between loads. This corresponds to 131 uncertain loads, and 21\% of the total system demand.  
%
\subsubsection{Polish 2383 Bus, Winter Peak Test Case }
We use the Polish Winter Peak Test Case with 2383 buses from Matpower 5.1 \cite{zimmermann2011}, with the following modifications. We set the lower generation limit to zero and increase the upper limit by a factor of 2. 
Many of the generators in the test case have very low (or even zero) reactive power capabilities. These generators are connected at PV buses were the voltage magnitude should be kept constant, but due to their lack of reactive power capability, they are not able to affect the voltage at their point of connection. Hence, these generators cannot keep the bus voltage constant during fluctuations, even for very small amounts of uncertainty, and the \ac{ccacopf} is always infeasible. To relieve this situation, we increase the upper and lower reactive power limits by +/- 10 MVAr for all generators.
All loads with consumption between 10 and 50~MW are assumed to be uncertain, with standard deviations equal to 10\% of the forecast and zero correlation between loads. This corresponds to 941 uncertain loads, and 67\% of the total system demand.  


\subsection{Investigated Approaches}
We compare several different versions of the \ac{ccacopf}, as well as different methods to solve them:
\begin{itemize}
    \item[\textbf{A}] \textbf{Standard AC OPF} without consideration of uncertainty.
    \item[\textbf{B}] \textbf{Iterative AC CC-OPF} is the iterative solution algorithm presented in Section \ref{sec:iterative}. We assume that $\alpha$ is pre-defined according to \eqref{eq:dg}, and that $\gamma$ is determined by the nominal (pre-defined) power factor of the uncertainty sources. We compare three different approaches to define the uncertainty margins:
    \begin{itemize}
        \item[\textbf{B1}] \textbf{Analytical} with uncertainty margins defined by the closed-form expressions \eqref{uncP} - \eqref{uncI}.
        \item[\textbf{B2}] \textbf{Monte Carlo} with empirical uncertainty margins obtained from a Monte Carlo simulation, as described in Section \ref{sec:alternative}.
        \item[\textbf{B3}] \textbf{Scenario Approach} with empirical uncertainty margins obtained from the limiting scenarios, as described in Section \ref{sec:alternative}.
    \end{itemize}
    \item[\textbf{C}] \textbf{One-Shot AC CC-OPF} is used to denote the solution obtained when solving \eqref{eq1} - \eqref{eq14} as a one shot problem. We compare both with pre-determined and optimized uncertainty response $\alpha,~\gamma$.
    \begin{itemize}
        \item[\textbf{C1}] \textbf{Fixed} $\boldsymbol{\alpha,\gamma}$ where $\alpha$ and $\gamma$ are pre-defined in the same way as for the iterative approach.
        \item[\textbf{C2}] \textbf{Optimized} $\boldsymbol{\alpha,\gamma}$ where $\alpha$ and $\gamma$ are co-optimized along with the generation dispatch.
    \end{itemize}
\end{itemize}



\subsection{Comparison of Solution Algorithms}
In the following, we compare the solutions obtained with the different solution approaches based on the analytical expressions for the uncertainty margins. Specifically, we use the deterministic AC OPF (A) as a benchmark, and solve the \ac{ccacopf} using the iterative approach (B1), the one-shot optimization with fixed participation factors $\alpha,\gamma$ (C1) and the one-shot optimization with $\alpha,\gamma$ as decision variables (C2). We compare the cost, the solution times and the number of iterations for the RTS96 and the 118 bus test cases. In order to fairly compare the computational times, the listed computational times are based on our own AC OPF implementations, which are based on functions available in Matpower and solved using KNITRO. The results are listed in Table \ref{table_algorithms}. The costs are shown relative to the deterministic AC OPF solution. 

{\begin{table} %[h!]
\caption{Cost of generation, solution time and number of iterations with different solution approaches. The numbers are for the IEEE RTS96 and IEEE 118 bus test systems.}
\label{table_algorithms}
\centering
\begin{tabular}{lllll}%{|l|c|c|c|c|}
%\hline
                & \textbf{Standard} & \textbf{Iterative} & \textbf{O-S Fixed}    & \textbf{O-S Opt}\\
                & \textbf{(A)}           & \textbf{(B1)}      & \textbf{(C1)}              & \textbf{(C2)} \\[+4pt]

\textbf{RTS96}           & & & & \\[+1pt]
~Cost            & \$36'771          & +7.7\%        & +7.6\%            & +3.2\%\\[+1pt]
~Time            & 1.5s              & 4.3s          & 4.3s              & 12.5s \\[+1 pt]
~Iterations      &                   & 4             &                   &  \\[+6 pt]
\textbf{118 Bus}         & & & & \\[+1pt]
~Cost            & \$3'504.1         & +1.9\%        & +1.9\%            & -\\[+1pt]
~Time            & 2min 5s           & 7min 46s      & 10min 51s         & - \\[+1pt]
~Iterations      &                   & 4             &                   &  \\
\end{tabular}
\end{table}}

As expected, the use of chance constraints in the \ac{ccacopf} formulations increases operational cost compared to the deterministic solution. When co-optimizing the participation factors $\alpha, \gamma$, the increase in cost is lower, as seen in previous chapters. 
While co-optimizing $\alpha, \gamma$ reduces cost, it also significantly increases computational time. For the 118 bus system, the optimization (C2) does not converge, even after running for 13h on a desktop computer.
To keep the computational time low and at least partially co-optimize $\alpha$, we can keep $\alpha$ as an optimization variable in the generation constraints (which are anyways linear in $\alpha$). Another option would be to pre-optimize $\alpha$ using, e.g., the DC CC-OPF from previous chapter.

We would like to note that the solution obtained with the iterative and one-shot solution approaches not only have the same cost, but also find the same optimal point (except for some very minor differences).




\subsection{Scalability}
To demonstrate how the iterative solution approach can be used with existing tools and scaled to large systems, we implement the iterative \ac{ccacopf} as an outer iteration on the standard Matpower ``runopf" function \cite{zimmermann2011} and solve the problem for all four test systems. The resulting times and the number of iterations are shown in Table \ref{table_solutions}. We also show the evolution of the generation cost between first, second and last iterations.

{\begin{table} %[h!]
\caption{Solution times, number of iteration and generation costs in the first, second and final iterations for different test cases. The problems are solved using the iterative approach (B1) with Matpower 5.1 and the default MIPS Solver.}
\label{table_solutions}
\centering
\begin{tabular}{lllll}%{|l|c|c|c|c|}
%\hline
                & \textbf{RTS96} & \textbf{118 Bus} & \textbf{300 Bus}  & \textbf{Polish}\\[+6pt]
Time            & 0.54s          & 1.15s            & 3.37s             & 31.89s\\[+4pt]
Iterations      & 5              & 4                & 5                 & 4 \\[+4pt]
Cost (1st)      & 36 771         & 3504.1           & 16 779            & 787 987\\
Cost (2nd)      & 40 249         & 3575.7           & 17 173            & 802 529\\
Cost (final)    & 40 127         & 3575.3           & 17 143            & 802 238\\
\end{tabular}
\end{table}}

The problems converge within 4-5 iterations. The overall problem solves very fast, and the solution is obtained within a few seconds for the smaller test systems and within half a minute for the Polish test case. 
Further, we observe that the main change in cost happens between the first and the second iteration, with only minor adjustments until final convergence. This implies that even if the problem should not converge, the intermediate iterations are typically also good approximations of the solution to the chance constrained problem.
Finally, we would like to note that Matpower with the default solver MIPS finds a slightly different optimal point than KNITRO, although the differences are quite minor. 





A  - deterministic
B1 - iterative with analytic margins
C1 - one-shot with fixed alpha
C2 - one-shot with optimized alpha

Results:
Focus only on cost and solution time
Comparison of fixed alpha vs. optimized alpha

        RTS96                               118bus
        Cost [\$]         Solution time     Cost [\$]         Solution time
A       36 771            1.5s (1.0s)       3504.1            2min 5s (50s)
B1      39 591 (+7.7\%)   4.3s (2.5s)       3569.9 (+1.9\%)   7min 46s (2min 6s)
C1      39 582 (+7.6\%)   4.3s              3569.6 (+1.9\%)   10min 51s                
C2      37 937 (+3.2\%)   12.5s             -                 -



Scalability
(note that the solution based on matpower finds a different solution than the above, as it uses a different solver)
                RTS96       118Bus      300Bus      Polish
Time            0.54s       1.15s       3.37s       31.89s
Iterations      5           4           5           4
Cost (1st)      36 771      3504.1      16 779      787 987
Cost (2nd)      40 249      3575.7      17 173      802 529
Cost (final)    40 127      3575.3      17 143      802 238


\subsection{Evaluation of Chance Constraint Reformulation}
The approximate \ac{ccacopf} has two main sources of inaccuracy that might lead to frequent overloads and violation of the chance constraint probability. First, the impact of uncertainty is approximated by a linear function, while it in reality depends on the full, non-linear AC power flow equations. Second, the analytical reformulation applied in this case study assumes a normal distribution, which might be an inaccurate description of the true uncertainty distribution. In the following case study, we investigate the performance of the analytical reformulation (B1) in terms of observed violation probabilities. We further compare the analytical reformulation (B1) with the sample-based methods to define the uncertainty margins, based on the empirical quantiles of the Monte Carlo approach (B2) and the uncertainty margins based on the scenario approach (B2). The comparisons are based on the RTS96 system, and the AC OPF within each iteration is solved using Matpower with MIPS.

\subsubsection{In-Sample Test of the Analytical Reformulation}
%With larger deviations, the linearized solution will increasingly deviate from the true solution. 
To assess how well the linearized model represents the actual impact of the uncertainty, we draw 10'000 samples from a multivariate normal distribution which matches the assumed distribution (i.e., we assume perfect knowledge of the distribution). Based on these samples, we assess the empirical violation probabilities through a Monte Carlo simulation. We perform the assessment for different standard deviations $\sigma_W=\{0.075, 0.1, 0.125\}$ and different acceptable violation probabilities $\epsilon_V=\epsilon_I=\{0.01, 0.05, 0.1\}$. 
Different values of the standard deviation $\sigma_W$ allow us to assess the performance of the method with fluctuations of different size, where larger standard deviations imply fluctuations further away from the linearization point.
With different violation probabilities $\epsilon$, we assess the accuracy of predictions for different parts of the distribution (smaller $\epsilon$ imply that we are further into the tail), and for quantiles that are closer (small $\epsilon$) or further (large $\epsilon$) away from the operating point.
%By varying $\sigma_W$ and $\gamma$, we assess how well the method performs for deviations of different size (different values of $\omega$) and different parts of the distributions (a smaller $\epsilon$ requires us quantiles that are further away from the operating point. 
The acceptable violation probabilities of the generator constraints on active and reactive power are kept constant at $\epsilon_P=\epsilon_Q=0.01$, as these constraints are not influenced by the non-linearities of the power flow equations. 

{\begin{table} %[h!]
\caption{In-sample testing of the performance of the analytical chance constraint reformulation (B1). The maximum empirical violation probability $\epsilon_{emp}$ observed for any individual chance constraint, as well as the number of samples with at least one constraint violation, corresponding to the joint violation probability. In the upper table, where $\sigma_W$ is varied, $\epsilon_I=\epsilon_V=0.01$. In the lower table, where $\epsilon=\epsilon_I=\epsilon_V$ is varied, $\sigma_W=0.1$.}
\label{insample}
\centering
\begin{tabular}{lccc}%{|l|c|c|c|c|}
%\hline
                    & $\sigma_W=0.075$ & $\sigma_W=0.1$ & $\sigma_W=0.125$ \\[+4pt]
Max. $\epsilon_{emp}$ & 0.011  & 0.013        & 0.017                \\[+3pt]
\# of Violated       & 647            & 650          & 812             \\
Samples             & (6.5\%)        & (6.5\%)      & (8.1\%)\\
& & & \\[+4pt]
                    & $\epsilon=0.01$ & $\epsilon=0.05$ & $\epsilon=0.1$ \\[+4pt]
Max. $\epsilon_{emp}$      & 0.013           & 0.044           & 0.092                \\[+3pt]
\# of Violated       & 650             & 1370            & 2194             \\
Samples             & (6.5\%)         & (13.7\%)        & (21.9\%)\\
                   
\end{tabular}
\end{table}}

The results of the in-sample testing are shown in Table \ref{insample}. If the analytical reformulation is accurate, the maximum empirical violation probability for a single chance constraint, denoted by $\epsilon_{emp}$ should be close to the desired violation probability $\epsilon=0.01$. 
The method performs quite well with the smallest standard deviation $\sigma_W=0.075$, but gets worse as the standard deviation increases. This is as expected, as the linearization becomes less accurate for larger deviations. 
We further observe that the method performs better for larger accepted violation probabilities $\epsilon=0.05$ and $0.1$. On the one hand, this might be because the quantiles corresponding to $\epsilon=0.05$ and $0.1$ are closer to the nominal operating point, in a region where the linearization is more accurate. On the other hand, a normal distribution might be a better approximation for the mid-part of the distribution than for the tails, hence providing better results when $\epsilon$ is not too small.

We further observe that the \ac{ccacopf} limits the total number of violated samples to a relatively small percentage, even though it only aims at enforcing the separate chance constraints. 



\subsubsection{Out-Of-Sample Test of the Analytical Reformulation}
The analytical reformulation assumes a normal distribution, while the true distribution of the forecast errors might be different. Therefore, we also include an out-of-sample test with uncertainty samples based on the historical data from APG described in Section \ref{sec:reformulationComparison}. We assign one set of historical samples, in total 8492 data points,  to each uncertain load. The samples are then rescaled to match the assumed standard deviation $\sigma_W$ and assumed correlation coefficient $\rho=0$. Since the number of available samples are limited, we base the Monte Carlo simulation on 5000 samples. 

The results of the out-of-sample testing based on APG historical data is shown in Table \ref{outofsample}. Again, the maximum empirical violation probability for a single chance constraint, denoted by $\epsilon_{emp}$ should be close to the desired violation probability $\epsilon=0.01$. 
We observe that the analytical reformulation based on the assumption of a normal distribution is still performing reasonably well, although the highest observed violation probability is 0.02 instead of 0.01.
Different from the in-sample testing, the magnitude of the standard deviation does not determine how well the method performs. However, we again observe that the method is better at enforcing the chance constraints with larger acceptable violation probabilities $\epsilon=0.05, 0.1$. 
The total number of violated samples is slightly higher than in the in-sample test, but remain in the same range.

{\begin{table} %[h!]
\caption{Out-of-sample testing of the performance of the analytical chance constraint reformulation (B1). The maximum empirical violation probability $\epsilon_{emp}$ observed for any individual chance constraint, as well as the number of samples with at least one constraint violation, corresponding to the joint violation probability. In the upper table, where $\sigma_W$ is varied, $\epsilon_I=\epsilon_V=0.01$. In the lower table, where $\epsilon=\epsilon_I=\epsilon_V$ is varied, $\sigma_W=0.1$.}
\label{outofsample}
\centering
\begin{tabular}{lccc}%{|l|c|c|c|c|}
%\hline
                    & $\sigma_W=0.075$ & $\sigma_W=0.1$ & $\sigma_W=0.125$ \\[+4pt]
Max. $\epsilon_{emp}$ & 0.017          & 0.014        & 0.020  \\[+2pt]
\# of Violated       & 374            & 369          & 461             \\
Samples             & (7.5\%)        & (7.4\%)      & (9.2\%)\\
& & & \\[+4pt]
                    & $\epsilon=0.01$ & $\epsilon=0.05$ & $\epsilon=0.1$ \\[+4pt]
Max. $\epsilon_{emp}$ & 0.014           & 0.054           & 0.093 \\[+2pt]
\# of Violated       & 369             & 724             & 1165             \\
Samples             & (7.4\%)         & (14.5\%)        & (23.3\%)\\
\end{tabular}
\end{table}}


\subsubsection{Comparison with Other Reformulations}

Finally, we compare the different iterative solution approaches (B1) with analytical uncertainty margins and $\epsilon=0.01$, (B2) with empirical uncertainty margins based on a Monte Carlo simulation and $\epsilon=0.01$, and (B3) with uncertainty margins based on the scenario approach and an acceptable joint violation probability of $\epsilon=0.1$. Within the optimization algorithm, we use 1000 samples to calculate the Monte Carlo margins, while the scenario approach prescribes the use of at least $N_S=2465$ samples. For the a-posteriori Monte Carlo simulation to evaluate the violation probabilities, we do an out-of-sample test using 5000 different samples from the historical data.

In Table \ref{table_joint}, the generation cost, solution time and number of iterations are listed. We also show the maximum empirical violation probability $\epsilon_{emp}$ and the total number of samples with violations. 
When comparing the cost of the solutions, as well as the empirical violation probabilities, it is important to remember that the sample-based solutions (B2) and (B3) depend on the samples that are drawn. If we would resolve the problem with a different set of samples, we would obtain a different solution. While we would like to check the solution by resolving it several times, we refrain from further simulations due to the limited amounts of available data and the large number of samples necessary for the scenario approach.

{\begin{table} %[h!]
\caption{Comparison of the iterative solution approach with (B1) analytical uncertainty margins and $\epsilon=0.01$, (B2) empirical uncertainty margins based on a Monte Carlo simulation and $\epsilon=0.01$, and (B3) uncertainty margins based on the scenario approach and an acceptable joint violation probability of $\epsilon=0.1$.}
\label{table_joint}
\centering
\begin{tabular}{llll}%{|l|l||c|c|}
%\hline
                    & \textbf{Analytical} & \textbf{Monte Carlo}  & \textbf{Scen. Approach}\\
                    & \textbf{(B1)}           & \textbf{(B2)}             & \textbf{(B3)} \\[+6pt]
Cost                & 40 127         & 39 922           & 41 455\\
                    & (+9.1\%)       & (+8.6\%)         & (+12.7\%)\\[+4pt]
Max. $\epsilon_{emp}$ & 0.014  & 0.019            & 0.003  \\[+4pt]
\# of Violated       & 369            & 502              & 35             \\
Samples             & (7.4\%)        & (10.0\%)         & (0.7\%)\\[+4pt]
Time                & 0.54s          & 2min 7s          & 6min 12s\\[+4pt]
Iterations          & 5              & 5                & 6 \\
\end{tabular}
\end{table}}

We observe that the analytical and Monte Carlo approaches lead to relatively similar solutions, although the Monte Carlo solution is lower. This decrease in cost does however come at the expense of higher violation probabilities and larger number of violated samples. It is interesting to see that the Monte Carlo approach, despite being calculated based on the full AC power flow equations and without any assumptions on the uncertainty distribution, actually performs worse than the analytical reformulation in terms of satisfying the upper limit on the violation probability $\epsilon_{emp}$ of the chance constraint. A larger number of samples could be used to obtain a better solution, but since we run a power flow for each sample in each iteration, a larger sample size would also increase computational time. The Monte Carlo already requires a lot more computational resources than the analytical reformulation, with a solution time of 2min 7s compared with 0.5s.

The scenario approach has a higher cost than the other two solutions, but also significantly lower violation probabilities. Actually, it oversatisfies the joint chance constraint by an order of magnitude. The limit on the acceptable, joint violation probability was set to $\epsilon_J=0.1$, whereas the empirical, joint violation probability is less than 1 \%. As a matter of fact, none of the solutions violates the limit on the joint probability, although the analytical and Monte Carlo approaches have lower cost. This shows one of the drawbacks of the scenario approach: While the solution guarantees feasibility of the chance constraint, the solution can be far from cost optimal. 
The sample bound for the scenario approach given in \cite{campi2009} is for general, convex problems. By using information about the specific structure of the problem, it might be possible to obtain tighter bounds that provide tighter bounds with fewer samples. However, as we have seen in Chapter \ref{Analytical_Reformulations}, it is hard to obtain a tight reformulation without assuming at least some properties of the underlying distribution. 

\fi






\iffalse
B1 - iterative with analytic margins
B2 - iterative with Monte Carlo margins
B3 - iterative with scenario approach margins

System: 118 bus

Samples: normal samples (in-sample test), APG samples (out-of-sample test)

For the in-sample test:
- analytic normal
- MC with 1000 samples
- scenario approach with XXX samples
-> make one set of samples to test from, then draw samples several times for the Monte Carlo and Scenario Approach

Record:
Violations per constraint
Number of samples that have any violations 
Cost



For the out-of-sample test:
- analytic normal
- analytic unimodal
- MC with 1000 samples
- scenario approach with XXX samples



\fi


\section{Conclusions}
In this chapter, we described an approximate formulation for the \ac{ccacopf}. The nominal operating point is represented using the full AC power flow equations, and the impact of uncertainty is accounted for through a linearization around the operating point. With the linearization, we can express the changes in voltage and current magnitudes, as well as active and reactive power production as linear functions of the fluctuations. This allows us to apply the previously presented analytical reformulation of the chance constraints, hence providing a reasonably accurate and tractable formulation of the \ac{ccacopf}. 

Different methods to solve the problem were proposed and discussed in the case study. The one-shot solution approach allow us to co-optimize the reaction to the fluctuations, which reduces cost, but also increases computational complexity. 
With the current implementation of the one-shot approach, the optimization did not converge for systems larger than the RTS96. However, improvements in the implementation and development of better solution algorithms can be expected to significantly improve computation time and scalability. 

As an alternative to the one-shot approach, we suggest an iterative solution method, where the chance constraints are enforced through an outer iteration on the deterministic AC OPF. The iterative solution method has several advantages. One the one hand, we are able to leverage the solution speed of existing, deterministic AC OPF solvers, which makes the problem easily scalable to large scale systems with a significant number of uncertainty sources. On the other hand, the iterative approach opens up for alternative definitions of the uncertainty margins, such as empricial evaluation based on a Monte Carlo simulation or the definition of uncertainty margins that allow us jointly enforce the chance constraints. 

In the case study, we assessed the performance of the method based on four test systems, the IEEE RTS96 system, the IEEE 118 bus and 300 bus systems, as well as the Polish Winter Peak test case with 2383 buses. For all test cases, a solution could be obtained within seconds to half a minute using the iterative solution approach with Matpower. The analytical reformulation based on the assumption of normally distributed uncertainty was shown to perform reasonably well in both in-sample and out-of-sample tests. In a comparison between the analytical reformulation, a Monte Carlo based reformulation and a reformulation based on the scenario approach, the analytical reformulation outperformed the Monte Carlo reformulation in terms of meeting the violation probability of the individual chance constraints, and the scenario approach in terms of cost.

































